How Scientists Use Jupyter Notebooks: Goals, Quality Attributes, and Opportunities

Computational notebooks are intended to prioritize the needs of scientists, but little is known about how scientists interact with notebooks, what requirements drive scientists' software development processes, or what tactics scientists use to meet their requirements. We conducted an observational study of 20 scientists using Jupyter notebooks for their day-to-day tasks, finding that scientists prioritize different quality attributes depending on their goals. A qualitative analysis of their usage shows (1) a collection of goals scientists pursue with Jupyter notebooks, (2) a set of quality attributes that scientists value when they write software, and (3) tactics that scientists leverage to promote quality. In addition, we identify ways scientists incorporated AI tools into their notebook work. From our observations, we derive design recommendations for improving computational notebooks and future programming systems for scientists. Key opportunities pertain to helping scientists create and manage state, dependencies, and abstractions in their software, enabling more effective reuse of clearly-defined components.

==> cleaned_up_results.tex <==
\subsection{Participants}
Out of the 20 participants, 7 had prior work experience in software engineering, 1 had formal training in software engineering, 6 knew the topic, and 6 had no knowledge at all.
%
\autoref{tab:participants} shows the participants' backgrounds.

\input{participant_table}

\subsection{Goals for Using Jupyter Notebooks}

\subsection{Emergent Software Quality Attributes}

\subsection{Notebook-Specific Usage Patterns}

==> tactics_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{List of Tactics}
\label{tab:tactics-list}
\begin{tabular}{@{}l@{}}
\toprule
Tactics                                                                      \\ \midrule
notebook modularity                                                          \\
notetaking                                                                   \\
abstraction                                                                  \\
enforcing linear execution                                                   \\
out of order execution                                                       \\
starting a fresh notebook to explore new ideas                               \\
restart and run all                                                          \\
adding empty cells                                                           \\
converting notebooks to scripts                                              \\
keeping imports at the top of a notebook                                     \\
keeping records of outputs outside notebook                                  \\
cell-based risk management                                                   \\
copying code from other notebooks                                            \\
copying code from scripts                                                    \\
deleting inspection code                                                     \\
execute code knowing there is an error                                       \\
managing data outside of notebook environment                                \\
storing notebooks alongside data                                             \\
converting a notebook to a PDF                                               \\
copying a notebook to compare the performance of two cells                   \\
create an empty notebook for debugging                                       \\
inspecting code in cleaned notebook over the current one                     \\
keep code out of functions                                                   \\
keeping code in comments                                                     \\
limiting the amount of times data needs to be loaded                         \\
maintaining notebook cleanliness                                             \\
overwriting inspection code                                                  \\
package management                                                           \\
reformatting to suit one's own preferences                                   \\
sectioning                                                                   \\
split cells based on their likelihood of recomputation and their performance \\
splitting a notebook to aid collaboration                                    \\
starting a fresh notebook for cleanup                                        \\
tracking cell execution progress                                             \\ \bottomrule
\end{tabular}
\end{table}
